Hypersparse Traffic Matrices from Suricata Network Flows using GraphBLAS

Hypersparse traffic matrices constructed from network packet source and destination addresses is a powerful tool for gaining insights into network traffic. SuiteSparse: GraphBLAS, an open source package or building, manipulating, and analyzing large hypersparse matrices, is one approach to constructing these traffic matrices. Suricata is a widely used open source network intrusion detection software package. This work demonstrates how Suricata network flow records can be used to efficiently construct hypersparse matrices using GraphBLAS.

==> Makefile <==
PAPERNAME = hpec2024-suricata-graphblas

all: clean ${PAPERNAME}.pdf
distclean: clean
tgz: all
	cd ..; \
	tar --exclude-vcs-ignores -czvf ${PAPERNAME}.tar.gz images/ tex/ 

%.pdf:  $(PAPERNAME).tex
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx
	pdflatex $<

clean:
	rm -f *.*~ *.log *.blg *.bbl *.aux *.out *.synctex.gz *.fdb_latexmk *.fls ${PAPERNAME}.pdf 




